SALSA: Sequential Approximate Leverage-Score Algorithm with Application in Analyzing Big Time Series Data

We develop a new efficient sequential approximate leverage score algorithm, SALSA, using methods from randomized numerical linear algebra (RandNLA) for large matrices. We demonstrate that, with high probability, the accuracy of SALSA's approximations is within $(1 + O({\varepsilon}))$ of the true leverage scores. In addition, we show that the theoretical computational complexity and numerical accuracy of SALSA surpass existing approximations. These theoretical results are subsequently utilized to develop an efficient algorithm, named LSARMA, for fitting an appropriate ARMA model to large-scale time series data. Our proposed algorithm is, with high probability, guaranteed to find the maximum likelihood estimates of the parameters for the true underlying ARMA model. Furthermore, it has a worst-case running time that significantly improves those of the state-of-the-art alternatives in big data regimes. Empirical results on large-scale data strongly support these theoretical results and underscore the efficacy of our new approach.

==> Acknowledgement.tex <==
\paragraph{Acknowledgment}

TBC

==> Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
TBC
% A novel approach has been introduced in this paper for the approximation of leverage scores of generic matrices. Influenced by the field of $\mathtt{RandNLA}$ and its applications in time series analysis, we have developed a novel sequential algorithm, named $\mathtt{SALSA}$, aimed at computing approximate leverage scores for big matrices. We have established analytical error bounds for this algorithm, and numerical experiments have shown its promising performance. Additionally, we have presented an application of $\mathtt{SALSA}$ in the domain of large-scale time series data. The $\mathtt{LSARMA}$ algorithm, a combination of various techniques, has been presented as an efficient and rapid approach for fitting $\mathtt{ARMA}$ models, with potential applications in the context of big time series datasets. We have proved the worst-case computational complexity of the $\mathtt{LSARMA}$ algorithm and validated its effectiveness through numerical experiments. For future research, we are interested in expanding our approach to the next level of generality in the realm of leverage score sampling, which involves developing an analogous algorithm for multivariate $\mathtt{VARMA}$ models.

